Attention Based Machine Learning Methods for Data Reduction with Guaranteed Error Bounds

Scientific applications in fields such as high energy physics, computational fluid dynamics, and climate science generate vast amounts of data at high velocities. This exponential growth in data production is surpassing the advancements in computing power, network capabilities, and storage capacities. To address this challenge, data compression or reduction techniques are crucial. These scientific datasets have underlying data structures that consist of structured and block structured multidimensional meshes where each grid point corresponds to a tensor. It is important that data reduction techniques leverage strong spatial and temporal correlations that are ubiquitous in these applications. Additionally, applications such as CFD, process tensors comprising hundred plus species and their attributes at each grid point. Reduction techniques should be able to leverage interrelationships between the elements in each tensor. In this paper, we propose an attention-based hierarchical compression method utilizing a block-wise compression setup. We introduce an attention-based hyper-block autoencoder to capture inter-block correlations, followed by a block-wise encoder to capture block-specific information. A PCA-based post-processing step is employed to guarantee error bounds for each data block. Our method effectively captures both spatiotemporal and inter-variable correlations within and between data blocks. Compared to the state-of-the-art SZ3, our method achieves up to 8 times higher compression ratio on the multi-variable S3D dataset. When evaluated on single-variable setups using the E3SM and XGC datasets, our method still achieves up to 3 times and 2 times higher compression ratio, respectively.

==> conclusion.tex <==








==> introduction.tex <==

Scientific research across various disciplines, from climate modeling, combustion analysis to particle physics, relies heavily on computational simulations and observational data \cite{jung2024application, gong2022region, golaz2019doe, chang2008spontaneous}. These simulations generate vast amounts of high-dimensional data, often exceeding the storage and processing capabilities of traditional computing systems \cite{chen2014big}. 
Therefore, effective data compression methods are crucial for efficiently handling, storing, and transmitting these vast datasets.

In scientific computing, lossy compression techniques hold significant importance, aiming to reduce data volume while retaining crucial attributes for analysis and interpretation. Unlike lossless compression, which strives for precise reconstruction, lossy compression methods trade some fidelity for increased compression ratios. Traditional lossy compression algorithms such as JPEG \cite{wallace1992jpeg}, MPEG \cite{boyce2021mpeg}, are widely used in the compression of multimedia data such as images, videos and audios. However, these algorithms doesn't fit for scientific data, which exhibit high dimensionality, irregular grid and complex spatiotemporal correlation. In the field of lossy compression for scientific data, numerous sophisticated techniques have emerged, each presenting unique strategies to achieve a fine-tuned balance between compression effectiveness and the preservation of fidelity. Among these, the SZ \cite{di2016fast,SZ1.4,SZ_3 } algorithms emerge as a standout candidate, renowned for its ability to compress scientific datasets effectively while ensuring the retention of crucial data.

In recent years, there has been remarkable progress in the application of machine learning techniques to data compression. For instance, in the domain of image compression, deep learning-based approaches such as Variational Autoencoders (VAEs) \cite{kingma2013auto} and Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} have demonstrated superior compression performance compared to traditional methods. While machine learning-based compression techniques have shown promise in multimedia domains, such as image and video compression, their application to scientific data types remains relatively unexplored. For instance, in climate modeling, combustion analysis, and particle physics, where data characteristics differ significantly from multimedia data, there is a lack of research on machine learning-based compression methods tailored to these domains.
The absence of a unified model for machine learning-based compression across multiple scientific data domains is a notable gap in current research. While individual studies have made significant strides in domain-specific compression, there is a need for a comprehensive framework that can adapt to diverse scientific datasets, including those with high dimensionality, irregular grids, and complex spatiotemporal correlations. Creating such a unified model for lossy compression of scientific data poses several challenges:

\begin{compactenum}

\item {\it High Dimensionality:} Scientific datasets are often characterized by high dimensionality, presenting challenges in effectively capturing and modeling complex dependencies and correlations within the data.
\item {\it Domain-specific Characteristics:} Various scientific domains possess distinct characteristics, data ranges, and distributions. Developing a compression model that can perform well across diverse domains is challenging, necessitating the model to capture domain-specific features and requirements.
\item {\it Error Bound Guarantee:} Ensuring error bounds in scientific data compression, especially for downstream analyses, poses a significant challenge. This involves not only achieving desired compression ratios but also maintaining fidelity to the original data within specified error margins, which are crucial for ensuring the reliability and accuracy of subsequent scientific analyses and interpretations.

\end{compactenum}


In this work, we propose a Guaranteed Unified Autoencoder (GUAE) to tackle the challenge of compressing data from multiple domains. Initially, the original data from various domains are segmented into high-dimensional tensor blocks. To ensure uniformity in data shape, we flatten these tensor blocks and pad them with zeros to create 1D vectors of consistent dimensions. We utilize graph convolution to capture correlations in multidimensional data, treating each element of the 1D vector as a node and constructing a graph based on inter-node correlations.

To maintain error bounds in the reconstructed data, we employ Principal Component Analysis (PCA) on the residual between the original and reconstructed data, obtaining a basis matrix for projecting each instance's residual. Coefficients are retained to facilitate accurate recovery, with their number incrementally increased until error bounds are satisfied. Quantization and entropy coding techniques are then applied to both the autoencoder's latent data and the PCA coefficients to improve compression ratios.

Furthermore, we assess the performance of GUAE by training it on three scientific datasets: S3D\cite{jung2024application}, E3SM\cite{golaz2019doe}, and XGC \cite{chang2008spontaneous}, representing different domains, using a single model. We compare GUAE's performance with that of ZS and domain-specific models, which only capture knowledge from one domain. The experimental results demonstrate that GUAE performs comparably to the domain-specific models. Compared to SZ \cite{SZ_3}, our method achieves significantly higher compression ratios while maintaining equal or lower reconstruction errors.

%


The remaining sections of the paper are structured as follows: Section ~\ref{sec:methodology} describes our unified model and compression pipeline. Experimental results are presented in Section~\ref{sec:experiment} for different levels of compression and comparison. Section~\ref{sec:relwork} presents related work. Conclusions are provided in Section~\ref{sec:conclusion}.






